The Loopix Anonymity System

We present Loopix, a low-latency anonymous communication system that provides bi-directional 'third-party' sender and receiver anonymity and unobservability. Loopix leverages cover traffic and brief message delays to provide anonymity and achieve traffic analysis resistance, including against a global network adversary. Mixes and clients self-monitor the network via loops of traffic to provide protection against active attacks, and inject cover traffic to provide stronger anonymity and a measure of sender and receiver unobservability. Service providers mediate access in and out of a stratified network of Poisson mix nodes to facilitate accounting and off-line message reception, as well as to keep the number of links in the system low, and to concentrate cover traffic. We provide a theoretical analysis of the Poisson mixing strategy as well as an empirical evaluation of the anonymity provided by the protocol and a functional implementation that we analyze in terms of scalability by running it on AWS EC2. We show that a Loopix relay can handle upwards of 300 messages per second, at a small delay overhead of less than 1.5 ms on top of the delays introduced into messages to provide security. Overall message latency is in the order of seconds - which is low for a mix-system. Furthermore, many mix nodes can be securely added to a stratified topology to scale throughput without sacrificing anonymity.

==> sections/bounces.tex <==
%\section{Bounces}

%\subsection{Message packet}

\ania{TODO: write about both MAC on header and on header + body}
The packet format which we are using to send the messages in our system is inspired and based on the Sphinx format~\cite{danezis2009sphinx}. 
First, we will present the Sphinx packet format and next, we present a new message format developed to allow to achieve some additional features.

\paragraph{Sphinx packet format}
Each message from Alice to Bob is encapsulated into the packet, which contains a header with meta-data, which we denote as ..., and an encrypted payload. Each header contains in itself the header for the next mix node. Let assume that each mix node amd each client in the nextwork has its unique key pair $\mathsf{(x_{i}, y_{i})}$.  
The header is defined by the following values:
\begin{itemize}
	\item $\mathsf{\alpha_{i}}  = g^{x_{A}b_{0}b_{1}\ldots b_{i-1}}$ and $b_{i} = \mathsf{h}(s_{i}, \alpha_{i})$,
	\item \BETA{i} = \ENC{s_{i}}{m_{i+1}, \beta_{i+1}, MAC_{i+1}}
	\item \MAC{i} = \FUNCTION{MAC}{s_{i}, \beta_{i}}.
\end{itemize}	
The message to be sent throught the network to the receiver is created as a layered encryption of the message $\mathsf{m}$, as
$\mathsf{E_{1}(E_{2}(E_{3}(...E_{N-1}(E_{R}(m)))))}$. 

\paragraph{New packet format description}
In the new packet format each message from Alice to Bob contains \emph{forward} \HF{i} and \emph{backward} \HB{i} headers and the layer encryption of the message. The forward header \HF{i}$= (\mathsf{\alpha_{i}}, \mathsf{\beta_{i}}, \mathsf{MAC_{i}})$ is defined by the following values
\begin{itemize}
	\item $\mathsf{\alpha_{i}}  = g^{x_{A}b_{0}b_{1}\ldots b_{i-1}}$ and $b_{i} = \mathsf{h}(s_{i}, \alpha_{i})$,
	\item \BETA{i} = \ENC{s_{i}}{m_{i+1},  cf_{i}, \beta_{i+1}, MAC_{i+1}}
	\item \MAC{i} = \FUNCTION{MAC}{s_{i}, \beta_{i}}.
\end{itemize}	  
In a similar way, the backward header is constructed as \HB{i} $= \mathsf{(\alpha_{i}^{B}, \beta_{i}^{B}, MAC_{i}^{B})}$, where \MAC{i}{B} = \FUNCTION{MAC}{s_{i}^{B}, \beta_{i}^{B}}, $\mathsf{\beta_{i}^{B}} = \mathsf{Enc}_{s_{i}^{B}}(m_{i-1}, \beta_{i-1}, \mathsf{MAC_{i-1}})$. \\
At the same time, when mix node $m_{i}$ processes the packet, it creates the backward header \HB on top of the previously received backward header. The message is encrypted using the keys shared among Alice and individual nodes and forwarded to Bob. At each step one of the encryption layers is removed and the message passed from the last mix node to Bob is only encrypted with Bob's public key. 

\paragraph{Packet processing} When the packet traverse mix node $m_{i}$ the following operations are conducted. First, mix node takes the element $\alpha_{i}$, which is used to compute the value of the shared sceret with Alica as \SECRET{i} $= \mathsf{\alpha_{i}}^{x_{i}}$. Next, node $m_{i}$ checks if the \MAC{i} is correct and decrypts value of the forward data \BETA{i} to obtain adress of the next mix node and values \CF{i}, \BETA{i+1}, \MAC{i+1} and updates the new header \HF{i+1} with these values.
The backward header is built at the time when the packet is traversing to Bob. Each mix node respectively adds a backward header, which will be used by this node if during the forwarding sending something will go wrong \ania{TODO}. 
Each mix node creates an element \ELEMENT{i}{B} in such a way that from a forward header extracts the value \CF{i} and computes \ELEMENT{i}{B} = $\alpha_{i}^{\text{cf}_{i}}$.

 \paragraph{Packet construction by Alice}
To construct the packet for message $m$ the individual values are computed by Alice as follows. 
At the beggining of the protocol Alice computes for each forward step an element \ELEMENT{i}{} $\in \mathbb{Z}$ which will be used to derive the shared secret between Alice and mix node $m_{i}$. Element \ELEMENT{}{} is created using Alice's secret key and obfuscated at each forward step by a blinding factor. Next, it is used to derive the shared secret between Alice and mix node $m_{i}$ as $s_{i} = $  \ELEMENT{i}{x_{i}}. Blinding factors are constructed as $b_{i} =$ \MAC{}$(s_{i}, \alpha_{i})$. Forward header contains also the message authentication code \MAC{i} $= \mathsf{MAC}(s_{i}, \beta_{i})$ and the encrypted informations \BETA{i} = \ENC{s_{i}}{m_{i+1},  cf_{i}, \beta_{i+1}, MAC_{i+1}}, where \CF{i} is a correction factor such that \CF{i} $= \prod_{j=i}^{2l-j+1}b_{i}$, $\forall_{1\leq i < l}$.  The correction factor \CF{i} is a multiplicative value of all blinding factors, which would be added to the element \ELEMENT{i}{} if the message came all way forward and backward to node $m_{i}$. Alice simulates also the backward path as if the message did the full circle traversing to and back from Bob and computs backward values of the element \ELEMENT{i}{B}, shared secret $s_{i}^{B}$ to evaluate the value \CF{i} and append to every forward header.  \\



==> sections/comparison_related.tex <==
\section{Comparison to Related Works}\label{sec:discussion}

\begin{xtoc}
\begin{itemize}
\item Hard comparison: Vuvuzilla, Herd (Druschel), Riposte (Maziers), Dissent (Ford), Hornet.
\item Relation to deployed systems: current Tor, LEAP Vpn, Ricochet.
\end{itemize}
\end{xtoc}

\subsection{Comparison with Vuvuzela}

\subsection{Comparison with Riposte}
\begin{itemize}
	\item In Riposte each client, who wants to send a message, has to submit a message of size proportional to the square root of the whole database making it unsuitable for sharing large messages among many clients.
	\item In Ripost they do not have a ``constant anonimity'' over time. Even assuming honest clients, when I'm sending a message I have to wait for some time when other people send their messages to build up an anonimity set. it can also cause a 'biase' - the lack of constant anonimity set may reveal that some groups are more likely to send/receive messages at a particular time.
	\item They have epochs,
	\item The three-server variant has a good efficiency, but requires two servers to be not compromised, whereas the s-server variant allows to achieve anytrust property, but is much less efficient.
	\item To deal with malicious servers, they have to use (1) a trusted non-colluding party , (2) use expensice ZKP.
	\item In case of whistelblowers, Riposte has to quarantee a large anonimity sets - which requires for example a long time of waiting to gather this set.
	\item Performance comparison (?)
\end{itemize}

==> sections/lookup_service.tex <==
\subsection{Lookup Service}

\begin{xtoc}
\begin{itemize}
\item Possible use for bounces / network status monitoring and statistics.
\item Used for presence in a central or distributed way.
\item Detection of reliability of mixes.
\item Lookup service for attachments.
\item Directory for keys: user keys (provider based PKI) or mixes (Provider based collective PKI?)
\item Propose the actual cryptographic lookup scheme.
\item Key idea: use anonymous channel + a weaker variant of PIR.
\end{itemize}
\end{xtoc}

==> sections/loopix_clientFig.tex <==
\newpage
\begin{center}
\begin{figure}[]
	\begin{tikzpicture}[font=\sffamily]
		\node[draw=none, fill=none] (sender) {\includegraphics[width=.1\textwidth]{users.png}};
		\node[draw=none, fill=none, right = of sender] (streamL) {};
		\node[draw=none, fill=none, above = of streamL] (streamP) {};
		\node[draw=none, fill=none, right = of streamL] (streamD) {};
		\node[draw=none, fill=none, right= of ]
	\end{tikzpicture}
\end{figure}
\end{center}

==> sections/message_formats.tex <==
\section{Message Packet Format}\label{sec:packet_format}

%\begin{xtoc}
%\begin{itemize}
%\item Traditional mix based format, using Public Key crypto at all hops, and without sessions (no symmetric keys left behind).
%\item Stateless on mixes despite replies, except for duplicate detection (SG-mix based timestamps? Possibly).
%\item Two headers, One forward, one constructed for backwards + Body.
%\item Properties: (not) can recognize bounce connected to message; (not) limited possibility for integrity protection backwards;
%\item Does not preclude partial checking.
%\end{itemize}
%\end{xtoc}
The traditional Chaum's design used \emph{public key encryption} to encapsulate messages. 
Senders layer encrypt each message and auxiliary meta information using mix nodes' public keys. Upon receiving a message each mix node decrypts it and extracts the \emph{header block} containing meta information about next entity to which pass the message. Next, each mix node adds a padding block of random bits to ensure that the message size is invariant to ensure \emph{bitwise unlinkability}. Finally, mix node batches the messages in a lexicographically order and sends them to the next destination.   
 
Using public key encryption allows an adversary, who gained the mix node secret key, to compromise all previous and future encryption. 
Moreover, this format does not protect against \emph{tagging} and \emph{reply} attacks.

In this section, we first briefly recall the Sphinx packet format~\cite{danezis2009sphinx} and next, describe the additional changes which Loopix introduces.
We apply the Sphinx packet format in our system, to ensure that the adversary is not able to gain any information from the observation of traversing packets, since the Sphinx packet format guarantees the unlinkability of the packets at each mixing step over the network. It also hides the overall path length and position of the mix server and provides the indistinguishable replies in form of \emph{Single Reply Blocks}.

\subsection{Sphinx packet format}

Each message wrapped into the Sphinx packet consists of two separate parts: a header $H$, the layers encrypted meta-data information for each stage of the traverse, and the payload $\rho$ of the message encapsulated as well into encryption. 
The header provides each mix server on the path with a confidential meta-data, which includes a single element of a cycling group, used to derive a shared encryption/decryption key, the routing information and the message authentication code which allows to verify if the header has not been modified by any malicious party.
In order to encode a message $\mathsf{m}$ sender $S_{i}$ pre-computes all session keys, shared with the mix servers on the path and uses them to encrypt the sequence of headers $H_{l-1}, \ldots, H_{0}$, where $H_{i}$ is defined as a tuple $(\alpha_{i}, \beta_{i}, \mathsf{MAC}_{i})$ and the message content. To compute the keys the sender picks a random value $x$ from a cyclic group of a prime order and computes a value $\alpha_{0} = g^{x}$. This value, called an \emph{element}, is used by each mix server $M_{i}$ to compute the key shared with the sender as $sh_{i} = \alpha_{i}^{x_{M_{i}}} = y_{M_{i}}^{x}$  and uses it to decrypt the received packet. To ensure the unlinkability of the packets' elements at each hop in the network, the element is blinded at each mixing step. The blinding factor is extracted from the shared secret by computing a keyed hash value $b_{i} = \mathsf{h}(\alpha_{i}, sh_{i})$ and the new output element is calculated as $\alpha_{i+1} = g^{xb_{0}\ldots b_{i}}$.  Thus, the sender is able to pre-compute all values to build a forward packet and each mix server, either mix node or provider, is able to reconstruct the corresponding shared secret. After computing the elements and shared keys, the sender creates a header $H_{i}$ destined for the $i'th$ mix node, in which the $\beta_{i}$ contains the following meta-data information:
\begin{itemize}
	\item $i+1$ - the address of the subsequent mix server, or the final destination of the message,
	\item $\mu$ - the delay after which the message should be sent,
	\item $dropFlag$ - the special flag informing the authorized party if this is a \emph{drop cover traffic} message (i.e., in \sysname this party is a randomly selected provider),
	\item $\beta_{i+1}$ - the meta-data designed for next entity on the path
\end{itemize} 
The message authentication code used for integrity protection is computed as \MAC{i} = \FUNCTION{MAC}{sh_{i}, \beta_{i}}. 
The Sphinx packet format requires some additional padding to be added during the construction and processing, in order to keep the length of the message invariant at each mixing stage, presented in details in~\cite{danezis2009sphinx}. 
After computing the headers, the sender creates the encrypted forward message by wrapping it into layers of symmetric encryption as $\rho_{i} = \mathsf{Enc}_{sh_{i}}(\rho_{i+1})$, where $\rho_{0}$ is the encryption of message $\mathsf{m}$ concatenated with the directory of the receiver $R_{j}$ and some additional padding.

The $i'th$ mix server after receiving the packet recomputes the shared key and checks if the $\mathsf{MAC}_{i}$ is correct. If not, the packet is dropped. Otherwise, the mix server decrypts the packet and extracts the header and checks the attached directory of the next entity and the delay. If the next entity will be another mix node or provider, $M_{i}$ computes a new output element $\alpha_{i+1}$ and schedules the packet to be send after the delay $\mu$. If the packet is processed by a provider and the forward address points to a client assigned to this provider and the \emph{dropFlag} is $0$, the provider stores the message in the client's inbox until the client retrieves it. If the \emph{dropFlag} is $1$, the provider drops the message.

%Senders encode a message by deriving all session keys, wrapping the message in multiple layers of encryption, and calculating the correct message authen- tication codes for each stage of the journey. Calculating the correct MACs is not a trivial task: the successive layers of padding that are encrypted at each stage of the mixing have to be included in the integrity check. The MACs ensure that a modified header is detected immediately.
%The payload of the message is kept separate from the mix header used to perform the routing. It is decrypted at each stage of mixing using a block cipher with a large block size (the size of the entire message), such as LIONESS [1]. In case the adversary modifies the payload in transit, any information contained in it becomes irrecoverable. Sender-anonymous messages contain the final address of the message, as well as the message itself as part of the payload, and so any modification destroys this information.

%Each message from sender \sender{i} to receipient \receiver{i} is encapsulated into the packet, which contains encrypted headers with meta-data, which we denote as \header{i}, and payload.
%Each header \header{i} contains within intself an encapsulated header \header{i+1} for the next mix node. The header for each hop is defined by the following values:
%\begin{itemize}
%	\item \ELEMENT{i} = $g^{x_{S_{i}} b_{0} b_{1} \ldots b_{i-1} }$ and $b_{i} = \mathsf{h}(s_{i}, \alpha_{i})$,
%	\item \BETA{i} = \ENC{s_{i}}{m_{i+1}, \beta_{i+1}, MAC_{i+1}},
%	\item \MAC{i} = \FUNCTION{MAC}{s_{i}, \beta_{i}}.
%\end{itemize}

%\paragraph{Packet construction}
%
%At the beggining of the protocol \sender{i} computes for each forward step a public element \ELEMENT{i} $\in \mathbb{Z}$ which will be used to derive the shared secret between Alice and mix node \Mixnode{i}. Element \ELEMENT{i} is created using sender's secret key $x_{S_{i}}$ and obfuscated at each forward step by a blinding factor in order to gurantee bitwise unlinkability. First, sender computes \ELEMENT{0} = $g^{x_{S_{i}}}$. Each blinding factor is calculated as $b_{i} =$  $\mathsf{h}(s_{i}, \alpha_{i})$
%Next, using \ELEMENT{i} sender computes the shared secrets with each mix node as \SECRET{i} = $\alpha_{i}^{x_{S_{i}}}$.

%\paragraph{Packet processing}



%\paragraph{Sphinx packet format}
%Each message from Alice to Bob is encapsulated into the packet, which contains a header with meta-data, which we denote as ..., and an encrypted payload. Each header contains in itself the header for the next mix node. Let assume that each mix node amd each client in the nextwork has its unique key pair $\mathsf{(x_{i}, y_{i})}$.  
%The header is defined by the following values:
%\begin{itemize}
%	\item $\mathsf{\alpha_{i}}  = g^{x_{A}b_{0}b_{1}\ldots b_{i-1}}$ and $b_{i} = \mathsf{h}(s_{i}, \alpha_{i})$,
%	\item \BETA{i} = \ENC{s_{i}}{m_{i+1}, \beta_{i+1}, MAC_{i+1}}
%	\item \MAC{i} = \FUNCTION{MAC}{s_{i}, \beta_{i}}.
%\end{itemize}	
%The message to be sent throught the network to the receiver is created as a layered encryption of the message $\mathsf{m}$, as
%$\mathsf{E_{1}(E_{2}(E_{3}(...E_{N-1}(E_{R}(m)))))}$. 
%
%\paragraph{New packet format description}
%In the new packet format each message from Alice to Bob contains \emph{forward} \HF{i} and \emph{backward} \HB{i} headers and the layer encryption of the message. The forward header \HF{i}$= (\mathsf{\alpha_{i}}, \mathsf{\beta_{i}}, \mathsf{MAC_{i}})$ is defined by the following values
%\begin{itemize}
%	\item $\mathsf{\alpha_{i}}  = g^{x_{A}b_{0}b_{1}\ldots b_{i-1}}$ and $b_{i} = \mathsf{h}(s_{i}, \alpha_{i})$,
%	\item \BETA{i} = \ENC{s_{i}}{m_{i+1},  cf_{i}, \beta_{i+1}, MAC_{i+1}}
%	\item \MAC{i} = \FUNCTION{MAC}{s_{i}, \beta_{i}}.
%\end{itemize}	  
%In a similar way, the backward header is constructed as \HB{i} $= \mathsf{(\alpha_{i}^{B}, \beta_{i}^{B}, MAC_{i}^{B})}$, where \MAC{i}{B} = \FUNCTION{MAC}{s_{i}^{B}, \beta_{i}^{B}}, $\mathsf{\beta_{i}^{B}} = \mathsf{Enc}_{s_{i}^{B}}(m_{i-1}, \beta_{i-1}, \mathsf{MAC_{i-1}})$. \\
%At the same time, when mix node $m_{i}$ processes the packet, it creates the backward header \HB on top of the previously received backward header. The message is encrypted using the keys shared among Alice and individual nodes and forwarded to Bob. At each step one of the encryption layers is removed and the message passed from the last mix node to Bob is only encrypted with Bob's public key. 
%
%\paragraph{Packet processing} When the packet traverse mix node $m_{i}$ the following operations are conducted. First, mix node takes the element $\alpha_{i}$, which is used to compute the value of the shared sceret with Alica as \SECRET{i} $= \mathsf{\alpha_{i}}^{x_{i}}$. Next, node $m_{i}$ checks if the \MAC{i} is correct and decrypts value of the forward data \BETA{i} to obtain adress of the next mix node and values \CF{i}, \BETA{i+1}, \MAC{i+1} and updates the new header \HF{i+1} with these values.
%The backward header is built at the time when the packet is traversing to Bob. Each mix node respectively adds a backward header, which will be used by this node if during the forwarding sending something will go wrong \ania{TODO}. 
%Each mix node creates an element \ELEMENT{i}{B} in such a way that from a forward header extracts the value \CF{i} and computes \ELEMENT{i}{B} = $\alpha_{i}^{\text{cf}_{i}}$.
%
%\paragraph{Packet construction by Alice}
%To construct the packet for message $m$ the individual values are computed by Alice as follows. 
%At the beggining of the protocol Alice computes for each forward step an element \ELEMENT{i}{} $\in \mathbb{Z}$ which will be used to derive the shared secret between Alice and mix node $m_{i}$. Element \ELEMENT{}{} is created using Alice's secret key and obfuscated at each forward step by a blinding factor. Next, it is used to derive the shared secret between Alice and mix node $m_{i}$ as $s_{i} = $  \ELEMENT{i}{x_{i}}. Blinding factors are constructed as $b_{i} =$ \MAC{}$(s_{i}, \alpha_{i})$. Forward header contains also the message authentication code \MAC{i} $= \mathsf{MAC}(s_{i}, \beta_{i})$ and the encrypted informations \BETA{i} = \ENC{s_{i}}{m_{i+1},  cf_{i}, \beta_{i+1}, MAC_{i+1}}, where \CF{i} is a correction factor such that \CF{i} $= \prod_{j=i}^{2l-j+1}b_{i}$, $\forall_{1\leq i < l}$.  The correction factor \CF{i} is a multiplicative value of all blinding factors, which would be added to the element \ELEMENT{i}{} if the message came all way forward and backward to node $m_{i}$. Alice simulates also the backward path as if the message did the full circle traversing to and back from Bob and computs backward values of the element \ELEMENT{i}{B}, shared secret $s_{i}^{B}$ to evaluate the value \CF{i} and append to every forward header.  \\
%


%\paragraph{Stop-and-go message format}
%
%The SG-mixes~\cite{kesdogan1998stop} are based on traditional mix networks, but the operating mix node is not batching the received messages in order to flush a fixed numer of them at once. Instead of that, the sender defines a specific delay $\mathsf{T_{i}}$ and time window $(\mathsf{T^{min}}, \mathsf{T^{max}})$ for every step of the circuit which the mix node is traversing. These two information are appended to the message packet and encrypted using mix nodes public keys. Every mix node in the SG-network after receiving the message decrypts it and extracts the time window and delay. Next, mix node checks if the arrival time of the message is within the time window. If it is not, the message is drooped. Otherwise, the mix node waits $\mathsf{T_{i}}$ units of time before sending it forward. SG-mix can be modeled as an $M/M/ \infty$ server with packet arrival rate $\lambda$ and service
%rate (delay rate) $\mu$. Any packet currently in the queue, regardless of position, is equally likely to be the next to depart the mix.

%\ania{To be continued}

%\subsection{Message Format with Bounces}
%
%\begin{xtoc}
%\begin{itemize}
%\item Key feature to implement higher level reliable delivery.
%\item As anonymous messages travel, a path is available backwards to signal failures or other network / user events (statistics, ...).
%\item Network signaling as well as end-user signaling feature.
%\item Possibly: the Providers may play a role in generating / consuming bounces.
%\end{itemize}
%\end{xtoc}
%
%\input{sections/bounces.tex}


==> sections/security_analysis.tex <==
%!Tex root = ../loopix.tex

\newcommand{\transmissions}{\ensuremath{\mathentity{T}}\xspace}
\newcommand{\trace}{\ensuremath{\mathentity{tr}}\xspace}
\newcommand{\powerset}{\raisebox{.15\baselineskip}{\Large\ensuremath{\wp}}}
\newcommand{\tracejoin}[1]{\ensuremath{\overset{#1}{\bowtie}}\xspace}

\newcommand{\ot}{\ensuremath{\leftarrow}\xspace}
 

\section{The proof of \sysname security}\label{sec:securityargument}

In this section we give a sound lower bound on the anonymity provided by Loopix against a GPA that collaborates with a subset of honest but curious mix servers. 


We refer to \Cref{sec:soundsimpleloopix} for the proof.

%%\sebastian{Idea: Mixes keep an output queue of size exactly $n'$. Whenever the mix holds less than $n'$ messages, it fills the queue with covert traffic. These covert messages are replaced by real messages as soon as they arrive. Mixes also have a secondary queue, dubbed the purgatory, in which additional messages are placed (if more than $n'$ messages reach the mix, so there are no covert messages to be replaced). }
%
%\sebastian{How do we call output channels in the rest of the paper?}
%
%\begin{definition}[Stronly Regular Mixes]\label{def:stronglyregularmixes}
%We say that a mix is \emph{strongly $\lambda$-regular}, if the frequency of its outputs to each other protocol party does not depend on its inputs. Formally, the frequency by which the mix sends messages on each \emph{output channel}, i.e., on each connection to other protocol parties, follows the distribution $\pois(\lambda)$ that is independent of the messages the mix receives.
%\end{definition}
%
%\subsection{Security Argument - Format}
%
%\begin{xtoc}
%\begin{itemize}
%\item Security argument based on a indistinguishability game. Definition. Proof either heuristic or very very formal (Markulf). Cannot link.
%\item Security argument for Providers being mostly untrusted.
%\item Cryptographic construction for general lookup. 
%\item Cryptographic construction around presence. Security definition / eval.
%\item Cryptographic arguments for the PKI based on providers.
%\end{itemize}
%\end{xtoc}
%
%\subsection{Security Against the Global Passive Adversary}
%
%\paragraph*{Assumptions}
%\begin{itemize}
%	\item We assume that the adversary is a global passive adversary, i.e., the adversary can observe all communication between protocol participants, but cannot compromise any protocol participants.
%	\item We only consider online senders. Technically, we assume that all senders are online.
%%	\item We only have indistinguishability for messages sent in the same epoch (as the timeouts leak the epoch)
%\end{itemize}
%
%\begin{theorem}[Anonymity against the GPA]\label{thm:gpa}
%Loopix has sender unobservability and sender-receiver tird-party unlinkability of $\delta$ against the global passive adversary, as by \Cref{def:anonymity}, where $\delta$ is negligible in the security parameter. \sebastian{We probably want to, at some point, have the AnoA definition for $\delta$.}
%\end{theorem}
%\begin{proof}
%We show the soundness of our sender unlinkability guarantees be the following two lemmas:
%
%\begin{lemma}\label{lemma:poissonoutput}
%The mix nodes and providers of Loopix are strongly $\lambda_M$-regular, as by \Cref{def:stronglyregularmixes}.
%\end{lemma}
%
%\begin{lemma}\label{lemma:direct-channels}
%Against an adversary that does not compromise protocol parties every connection between users, providers and mix nodes can be replaced by a direct channel without harming the success of the adversary.
%\end{lemma}
%
%\begin{proof}[Proof for \Cref{lemma:poissonoutput}]
%As described in \Cref{section:mixnode-formal}, each message arriving in a mix node \mixnode is delayed for a time \delayTi and then put into the respective output queue $\outputqueue{j}$ for the intended recipient $\mixnode_j$. \sebastian{Sanity check: make sure we described this.}
%
%By construction, every mix node \mixnode outputs a message to any other mix node/provider $\mixnode_j$ if and only if it has an output queue $\outputqueue j$ for that mix node/provider. Moreover, a message is sent if and only if the respective poisson process $\pois(\lambda_M)$ requires \mixnode to send a message. The frequency by which messages are sent is thus completely independent of the inputs the mix node receives.
%\end{proof}
%
%\begin{proof}[Proof for \Cref{lemma:direct-channels}]
%Let $\adv$ be an adversary that can observe the whole network.
%Recall the protocol as it is specified in~\Cref{section:architecture} within the AnoA game in which the adversary $\adv$ gives to the challanger the \emph{input} messages, on which she has a full control over which senders send particular messages to which receivers. Moreover, \adv gives the challanger \Chal a \emph{challange} tuple, defined as $ (S_{0}, S_{1}, R_{0}, R_{1}, m)$. The challanger \Chal applies the anonymity function, i.e., for sender unobservability chooses one sender $S_b \in \set{S_0,S_1}$ depending on the challenge bit $b$ and instructs this sender $S_b$ to send a message $m$ to $R_0$.
%After the observation $\adv$ outputs a bit $b^*$. If it is equal to the challange bit $b$, $\adv$ wins the game.
%
%We now construct an adversary $\bdv$ that does not observe any part of the network and that still achieves the same advantage $\delta$ in the game as $\adv$.
%
%\bdv starts by generating keys for all honest parties and distributes them in the same fashion as the original protocol. \bdv internally runs \adv. For every connection between protocol parties, \bdv behaves as follows, depending on the type of the connection:
%\begin{itemize}
%	\item For every user $S$: \bdv generates \emph{local noise packets} \noisepacket using the same poisson distributions that users use for sending their messages. \bdv lets \adv observe these packets between $S$ and \provider. Moreover, $\bdv$ generates local noise packets \noisepacket following the distribution by which users fetch messages from their inboxes, as well as local noise packets \noisepacket for the respective answers.
%	\item For every mix node/provider \mixnode: \bdv simulates \mixnode without any input messages. Consequently, \mixnode will only send local noise packets \noisepacket to all connected mixnodes/providers $\mixnode'$ following the distribution $\pois(\lambda_M)$.
%\end{itemize}
%When \adv finally outputs its guess for the challenge bit $b^*$, \bdv also outputs $b^*$.
%
%We now show that $\adv$ cannot distinguish whether it is within the real game (with the challenger, and observing real messages) or whether it is being simulated by $\bdv$ (except with negligible probability).
%
%We first note that for the GPA, real message packets are indistinguishable from a \emph{local noise packet} generated by \mixnode, which follows from \sebastian{@Ania: whereever we discuss the leakage of the message packet format}.
%
%We distinguish the following observations $\adv$ can make:
%\begin{itemize}
%	\item A user sends messages to its provider: All users send messages to their provider following three distributions $\pois(\lambda_L)$ for sending loops, $\pois(\lambda_D)$ for sending drop cover messages, and $\pois(\lambda_P)$ for sending actual messages. $\bdv$ knows $\lambda_L,\lambda_D,$ and $\lambda_P$ (as they are publicly known) and sends messages following the distribution $\pois(\lambda_L+\lambda_D+\lambda_P)$, which is the same distribution used by the actual user. Since $\adv$ cannot distinguish real message packets from local noise packets, it cannot distinguish between messages sent from users to their provider and simulated user messages created by \bdv.
%	\item A user fetches messages from its provider: All users regularly send messages to fetch messages from their inbox. Recall that these messages are sent regularly, following the same frequency and upon receiving a message from a user to fetch messages from their inbox, providers always send the same number of messages back in return. Consequently, since $\adv$ cannot distinguish real message packets and their responses from local noise packets, it cannot distinguish between fetch messages from the user with corresponding results from the provider and and simulated user provider interactions created by \bdv.
%	\item A mix node/provider sends messages to another mix node/provider: By \Cref{lemma:poissonoutput} both mix nodes and providers are strongly $\lambda_M$-regular as in \Cref{def:stronglyregularmixes}. Consequently, the frequency by which they send messages to all other connected mix nodes/providers follows a distribution $\pois(\lambda_M)$, which is exactly the same frequency by which the mixes and providers simulated by $\bdv$ send local noise packets. Since $\adv$ cannot distinguish real message packets local noise packets, it cannot distinguish the messages sent by real mix nodes/providers and the simulated messages created by \bdv.
%\end{itemize}
%
%Thus, there is an adversary $\bdv$ that achieves the same advantage as $\adv$, but that does not observe any communication.
%\end{proof}
%
%We have shown that we can analyze a game in which the communication between entities is replaced by direct channels. Since the global passive adversary by definition does not compromise any protocol parties, it is effectively blind in this game and thus has an advantage of $0$. Both lemmas introduce a negligible error, leaving us with an adversary that has only a negligible advantage $\delta$ as by \cref{def:anonymity}. 
%
%This concludes the proof for sender unobservability of \Cref{thm:gpa}. 
%The proof for sender-receiver third-party unlinkability follows analogously.
%\end{proof}
%
%\subsection{Security Against Malicious Protocol Parties}
%For quantifying the anonymity that Loopix provides in light of malicious protocol parties we introduce a simplified model of Loopix.
%
%\begin{definition}[\TTP-Loopix]\label{def:ttp-loopix}
%Instead of sending packets through the network of mixes, we introduce a \emph{trusted third party} (\TTP) that manages the content of all communication. 
%
%Instead of sending packets, protocol parties send \emph{handles} to each other, effectively ensuring perfect cryptography, whereas the \TTP handles all the messages and the auxiliary meta-information. Protocol parties no longer require keys, but are assumed to be connected to the \TTP by a direct, unobservable channel. To obtain information about the forwarded messages, such as where a particular message should be destinated in the next hop or the required delays, the entities contact \TTP directly.
%
%Every sender, say, Alice, generates handles $\{h_0, \ldots, h_n\}$ as random nonces, where $n$ is the length of the path. Next, she sends a tuple $(h_i, \mixnode_i, (\mixnode_{i+1}, \delayTi))$, for every $i \in \{0, \ldots, n-1\}$ to the \TTP, where $\mixnode_i$ specifies the mix node/provider is allowed to look up the handle, $\mixnode_{i+1}$ specifies the mix node/provider to which $\mixnode_i$ is to forward the message and $\delayTi$ specifies a time delay which $\mixnode_i$ has to wait before forwarding the message. Finally, Alice sends also a tuple $(h_n, B, m)$ to the \TTP, where $m$ is the message she wants to send to the recipient $B$. Each tuple is stored by the \TTP in a database.
%
%Upon receiving a request \fetch{h_{i}} to the \TTP from any protocol participant $P$ (either a mix node/provider or a recipient), the \TTP checks whether the database stores entry $(h_{i}, P, X)$, where $X$ contains information about the next entity to which the message should be forwarded and the delay. If so, the \TTP sends $X$ to $P$.\\
%\end{definition}
%
%The following lemma ensures that the simplified model of Loopix faithfully considers all passive attacks.
%\begin{lemma}
%Let $M$ be a set of mix nodes, providers and users.
%
%If \TTP-Loopix as defined in \Cref{def:ttp-loopix} has sender unobservability, receiver unobservabiliry or sender-receiver tird-party unlinkability of $\delta$ against any adversary $\adv$ that (additionally to being the GPA) compromises all protocol parties in $M$, then Loopix has sender unobservability, receiver unobservabiliry or sender-receiver tird-party unlinkability of $\delta+\mu$ against any adversary $\adv$ that (additionally to being the GPA) compromises all protocol parties in $M$, where $\mu$ is negligible in the security parameter.
%\end{lemma}
%\begin{proof}
%The coarse strategy of the proof is as follows. The packet format does not leak any information about the payload to the GPA that just observes the communication. By observing the network the adversary can only learn which party sends a message to which other immediate party. Mix nodes only learn the limited meta-data information that they need for processing the message, but do not learn anything beyond that.
%
%By \Cref{lemma:packet} \sebastian{@Ania: reference to where we show stuff about the packet format}
%whenever an adversary \adv observes a packet from a protocol participant $P$ to another protocol participant $P'$, s.t. $P'$ is not compromised by \adv cannot distinguish between whether this packet is a real message packet or a \emph{local noise packet} generated by $P$.
%
%\sebastian{@Ania: can we show that the auxiliary information is indistinguishable from pure randomness or something like that?}
%
%Malicious mix nodes/providers additionally only learn next entity and the message delays, as well as the time at which the messages are sent.
%
%We show the lemma via a reduction proof. Given any adversary $\adv$ against Loopix, we construct an adversary $\bdv$ against \TTP-Loopix that compromises the same entities and that achieves the same advantage (up to a negligible difference). Consequently, if we can show that for all adversaries $\bdv$ compromising a set $M$ of entities against \TTP-Loopix the advantage is bounded by $\delta$, then the advantage of any adversary \adv compromising the same set $M$ of entities is bounded by $\delta+\mu$, where $\mu$ is negligible.
%
%Given any adversary \adv, we construct an adversary \bdv as follows:
%\bdv starts by generating keys for the adversary and for all honest parties and distributes them in the same fashion as the original protocol. 
%\bdv internally runs \adv. Whenever \adv wants to compromise any mix node $M$, \bdv tries to compromise the same mix node.
%Whenever \bdv observes a handle $h_{i}$, it conducts a specific action depending on where it observes the handle:
%\begin{itemize}
%	\item If \bdv observes it on a link, without controlling either the sender or the recipient of the handle, it generates an encryption of a random message that is of the same length as a packet.
%	\item If the recipient of the handle $P_0$ is compromised, let $(P_0, \ldots, P_k)$ be the list of all following compromised parties on the path. \bdv fetches, for each handle $\{h_0, \ldots, h_k\}$, the respective information from the \TTP and then creates a packet as follows:
%	\begin{itemize}
%		\item If $P_k$ is a recipient: Upon sending \fetch{h_k}, \bdv receives the payload message $m$. Subsequently it creates a package with payload $m$.... \sebastian{Add the package creation functions here. the package has to be creates as if it was just going to be sent to and decrypted by $P_0, \ldots, P_{k-1}$}
%		\item If $P_k$ is a provider or a mix node: \bdv creates a package with a random payload... \sebastian{Add the package creation functions here. the package has to be creates as if it was just going to be sent to and decrypted by $P_0, \ldots, P_{k}$}
%	\end{itemize}
%	\item If a (sending) user is compromised, \bdv creates the handles honestly, but additionally creates a correct mix packet (and forwards it to \adv). If \bdv later observes a handle it registered at the \TTP, instead of generating a fresh packet, it presents to \adv the (processed) packet that would have been observed on the way. \sebastian{I think we don't consider (passively) malicious users at this point, but I wanted to note the steps necessary for modeling them anyway.}
%\end{itemize}
%When \adv finally outputs its guess for the challenge bit $b^*$, \bdv also outputs $b^*$.
%
%Since the games are equal in terms of the challenge bit and the victory condition of the adversary, \bdv wins in $G_1$ if and only if $\adv$ outputs the correct challenge bit. We conclude the proof by showing that for $\adv$ the games $G_0$ and the simulated game with $\bdv$ in $G_1$ are computationally indistinguishable.
%
%Whenever \adv in $G_0$ observes a message and controls neither sender nor recipient, it cannot distinguish the (end-to-end encrypted) communication from a freshly generated random encryption. \sebastian{We might want to use the encryption keys of the parties, if they have long time keys, or we might have to simulate a key handshake.}
%
%\sebastian{As soon as we have the packet creation functions fixed, argue why we do a perfect simulation here.}
%\end{proof}
%
%\sebastian{Now we should do some quantifications, following the ``probability of message to arrive within delay'' idea.}
%
%\begin{algorithm}
%Probabilty space $\Omega_{n,k}^p$, for stratified topology ($n$ mix nodes per stage) and for a path length of $k$:
%\begin{algorithmic}
%	\STATE $\mixnode_1, \mixnode_1', \ldots, \mixnode_k, \mixnode_k' \randomfrom \set{1, \ldots, n}$
%	\STATE $d_A, d_B, d_0, d_0', d_1,d_1', \ldots, d_k, d_k' \from $ ExpDist.
%	\STATE $c_0, c_0', c_1,c_1', \ldots, c_k, c_k' \randomfrom \set{\mathstring{True},\mathstring{False}}$
%	\FOR{$i \in [1, \ldots, k]$}
%		\IF{$\mixnode_i = \mixnode_i'$}
%			\STATE $c_i' := c_i$
%			\STATE $d_{i-1}^{\mathstring{fake}} := d_{i-1}$
%			\STATE $d_{i-1}'^{\mathstring{fake}} := d'_{i-1}$
%		\ELSE
%			\STATE $d_{i-1}^{\mathstring{fake}} \from $ ExpDist.
%			\STATE $d_{i-1}'^{\mathstring{fake}} \from $ ExpDist.
%		\ENDIF
%	\ENDFOR
%	\FOR{$i \in [0, \ldots, k]$}
%		\STATE $D_i := d_A + d_0 + d_1 + \ldots  + d_i$
%		\STATE $D'_i := d_B + d'_0 + d'_1 + \ldots  + d'_i$
%		\STATE $DF_i := d_A + d_0 + d_1 + \ldots  + d_{i-1} + d_{i}^{\mathstring{fake}}$
%		\STATE $DF'_i := d_B + d_0' + d_1' + \ldots  + d_{i-1}' + d_{i}'^{\mathstring{fake}}$
%	\ENDFOR
%\end{algorithmic}
%\caption{Probability space as required by \Cref{thm:mixnodeadv}.}
%\label{alg:probspace}
%\end{algorithm}
%
%For reasoning about malicious protocol participants we define a large probability space modeling two mix paths, one initiated by a user Alice $(\mixnode_1, \mixnode_2, \ldots, \mixnode_k)$ and one by another user Bob $(\mixnode'_1, \mixnode'_2, \ldots, \mixnode'_k)$, modeling either the two challenge messages (for sender-receiver third party unlinkability) or the challenge message sent by one user and a cover message sent by the other user. We sample the delays these messages should wait in the mix nodes from the exponential distribution, where $d_A$ describes the delay of Alice, and $d_B$ the delay of Bob, i.e., delays to sending the messages in the first place, $d_0$ and $d'_0$ describe the delays of Alice's and Bob's provider for the given message and $d_i$ and $d'_i$ describe the delays the messages wait in mix nodes $\mixnode_i$ and $\mixnode'_i$ respectively. We randomly draw a boolean flag $c$, describing whether a provider is compromised ($c_0=\mathstring{True}$ or $c'_0=\mathstring{True}$) or whether a mix node is compromised ($c_i=\mathstring{True}$ or $c'_i=\mathstring{True}$ for mix nodes $\mixnode_i$ and $\mixnode'_i$). 
%Furthermore, we define the delay $D_i / D'_i$ the messages have experienced in the first $i$ steps as the sum of the delays up to that point. As the adversary cannot, for honest mix nodes, distinguish outgoing messages, we define a theoretical, fake delay $DF_i / DF'_i$ to describe the delay for the first $i-1$ steps plus one additional delay of another message from $\mixnode_i$ to $\mixnode'_{i+1}$ (for $DF_i$) or from $\mixnode'_i$ to $\mixnode_{i+1}$ for $DF'_i$.
%We refer to \cref{alg:probspace} for a formal description of this probability space and now utilize it for our theorem against compromised mixes. 
%
%\begin{theorem}\label{thm:mixnodeadv}
%Against an adversary that compromises mix nodes with probability $p$ we define the probability space of the game as $\Omega_{n,k}^p$ as in \Cref{alg:probspace}. Against such an adversary, even in collaboration with the challenge recipient, Loopix has a sender unobservability of $\delta$ with
%\[\small
%	\delta = 1 - \condpr{\begin{aligned}
%&(\lnot c_0' \lor \mixnode_1=\mixnode_1') \land \lnot c_1 \land D_1 > DF_0'\\
%\lor &(\lnot c_1' \lor \mixnode_2=\mixnode_2') \land \lnot c_2 \land D_2 > DF_1'\\
%\lor &\quad\dots\\
%\lor &(\lnot c_{k-1}' \lor \mixnode_k=\mixnode_k') \land \lnot c_k \land D_k > DF_{k-1}'\\
%\end{aligned}}{\Omega_{n,k}^p}
%\]
%
%\end{theorem}
%\begin{proof}[proof sketch]
%\sebastian{Some explanation on what we are doing and why we think it's not just a good idea, but it captures the anonymity Loopix provides.}
%
%We user the following reasoning for calculating these guarantees:
%\begin{itemize}
%	\item We consider the path of the challenge message and the path of one message the alternative user sends and check whether those messages could meet (or appear to meet).
%	\item Whether or not the messages meet depends on their delays. If the delays of the challenge message are large, the challenge message could meet a lot of possible other messages as well and we assume it to be safe. If the delays of the challenge message make it impossible to meet the alternative message (because the alternative message had not arrived yet), the adversary may win the game. This distinction makes sense only because the adversary can know (for sure) when the challenge message arrives, by compromising the recipient. However, it does not know when the alternative message arrives, if this alternative message has visited at least one honest mix in the process (the probability of this not happening is $p^{k}$ and none of the clauses for the messages meeting would be fulfilled).
%	\item As soon as those messages meet (or could have met) within the same (honest) mix node, the adversary cannot win anymore.
%	\item As soon as the alternative message is in an honest mix in step $i-1$ and a message from this mix reaches the mix $\mixnode_i$ in which the challenge message currently is, from the adversary's perspective, this is indistinguishable to the challenge message and the alternative message meeting in the honest mix $\mixnode_i$. Consequently, the adversary cannot win anymore.
%\end{itemize}
%
%In an (honest) mix $\mixnode_{i-1}'$ the delay by which the next message is sent on the outgoing channel to $\mixnode_i$ is equally distributed as the other delays. Since we assume that the adversary does not control sending users, we can assume that the delay is unknown to the adversary (no matter whether the message is a loop message, a cover message to a random recipient sent by a user or a local noise message from one mix to another). Because of the self-similarity of the exponential distribution of delays, we can consider the remaining delay as a fresh delay drawn from the exponential distribution. We label this virtual delay with $d_{i-1}^{\mathstring{fake}}$. If the message from Bob is actually sent to mix $\mixnode_i$ (if we have $\mixnode_i' = \mixnode_i$), we use the real delay $d_{i-1}'$ specified by Bob instead.
%\end{proof}
%
%
%\begin{theorem}\label{thm:mixnodeadv-sr}
%Against an adversary that compromises mix nodes with probability $p$ we define the probability space of the game as $\Omega_{n,k}^p$ as in \Cref{alg:probspace}. Against such an adversary, even in collaboration with both challenge recipients, Loopix has a sender receiver unlinkability of $\delta$ with
%\[\small
%	\delta = 1 - \condpr{\begin{aligned}
%\Big(& (\lnot c_0' \lor \mixnode_1=\mixnode_1') \land \lnot c_1 \land D_1 > DF_0'\\
%\lor &(\lnot c_1' \lor \mixnode_2=\mixnode_2') \land \lnot c_2\land D_2 > DF_1'\\
%\lor &\quad\dots\\
%\lor &(\lnot c_{k-1}' \lor \mixnode_k=\mixnode_k') \land \lnot c_k \land D_k > DF_{k-1}' \Big)\\
%&\quad\land\\
%\Big(&(\lnot c_0 \lor \mixnode_1=\mixnode_1') \land \lnot c_1' \land D_1' > DF_0\\
%\lor &(\lnot c_1 \lor \mixnode_2=\mixnode_2') \land \lnot c_2' \land D_2' > DF_1\\
%\lor &\quad\dots\\
%\lor &(\lnot c_{k-1} \lor \mixnode_k=\mixnode_k') \land \lnot c_k' \land D_k' > DF_{k-1}\Big)\\
%\end{aligned}}{\Omega_{n,k}^p}
%\]
%
%\end{theorem}
%\begin{proof}
%The proof follows analogously to the proof of \Cref{thm:mixnodeadv}, the only difference being that we keep track of both messages and either they directly meet or they could have met.
%\end{proof}
%
%
%
%%\begin{figure}
%%\begin{tikzpicture}
%%\begin{axis}[
%%xlabel={Percentage of corruption},
%%xlabel style={text width=7.5cm}, 
%%ylabel style={font=\large}, 
%%ylabel={Adversarial advantage $\delta$},
%%legend style={cells={align=right},at={(.65,1.1)}},
%%legend columns=2,
%%legend entries={5-diff,5-same,10-diff,10-same,20-diff,20-same,50-diff,50-same,100-diff,100-same},
%%%symbolic x coords={sa,ra,rel},
%%%	ybar=1.5,
%%%	xtick = data,
%%%	xticklabels={},
%%%	xtick style={draw=none},
%%	xmin=0,
%%	xmax=100,
%%	ymin=0,
%%	ymax=1,
%%%	bar width=2,
%%%	enlarge x limits=.20,
%%	unbounded coords=discard,
%%%	boxplot/draw direction=y,
%%	%width=\graphwidth,
%%	%height=\graphheight,
%%]
%%%SA
%%\addplot[style={draw=red}, line width=1] table [col sep=comma] {sim/graph-pathlength-5-provider-False.csv};
%%\addplot[dotted, style={draw=red}, line width=1] table [col sep=comma] {sim/graph-pathlength-5-provider-True.csv};
%%\addplot[style={draw=green}, line width=1] table [col sep=comma] {sim/graph-pathlength-10-provider-False.csv};
%%\addplot[dotted, style={draw=green}, line width=1] table [col sep=comma] {sim/graph-pathlength-10-provider-True.csv};
%%\addplot[style={draw=blue}, line width=1] table [col sep=comma] {sim/graph-pathlength-20-provider-False.csv};
%%\addplot[dotted, style={draw=blue}, line width=1] table [col sep=comma] {sim/graph-pathlength-20-provider-True.csv};
%%\addplot[style={draw=black}, line width=1] table [col sep=comma] {sim/graph-pathlength-50-provider-False.csv};
%%\addplot[dotted, style={draw=black}, line width=1] table [col sep=comma] {sim/graph-pathlength-50-provider-True.csv};
%%\addplot[style={draw=yellow}, line width=1] table [col sep=comma] {sim/graph-pathlength-100-provider-False.csv};
%%\addplot[dotted, style={draw=yellow}, line width=1] table [col sep=comma] {sim/graph-pathlength-100-provider-True.csv};
%%\end{axis}
%%\end{tikzpicture}
%%\caption{A plot of the adversarial advantage against sender unobservability depending on the percentage of compromised mixes. We display one graph per length of the path of mixes. The graphs assume that we have a stratified network topology with $10$ mix nodes per stage and each mix is compromised at random with a probability $p$ equal to the percentage of corruption. The challenge users use different providers (or a compromised provider) (solid lines) or the same uncompromised provider (dotted lines).}\label{fig:compromisedmixplot}
%%
%%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{sections/graphs/security_graph1.pdf}
%\caption{\small{A plot of the adversarial advantage against sender unobservability depending on the percentage of compromised mixes. We display one graph per length of the path of mixes. The graphs assume that we have a stratified network topology with $10$ mix nodes per stage and each mix is compromised at random with a probability $p$ equal to the percentage of corruption. The challenge users use different providers (or a compromised provider) (solid lines) or the same uncompromised provider (dotted lines).}}
%\label{fig:compromisedmixplot}
%
%\end{figure}
%
%%\begin{figure}
%%\begin{tikzpicture}
%%\begin{axis}[
%%xlabel={Percentage of corruption},
%%xlabel style={text width=7.5cm}, 
%%ylabel style={font=\large}, 
%%ylabel={Adversarial advantage $\delta$},
%%legend style={cells={align=right},at={(.65,1.1)}},
%%legend columns=2,
%%legend entries={5-diff,5-same,10-diff,10-same,20-diff,20-same,50-diff,50-same,100-diff,100-same},
%%%symbolic x coords={sa,ra,rel},
%%%	ybar=1.5,
%%%	xtick = data,
%%%	xticklabels={},
%%%	xtick style={draw=none},
%%	xmin=0,
%%	xmax=100,
%%	ymin=0,
%%	ymax=1,
%%%	bar width=2,
%%%	enlarge x limits=.20,
%%	unbounded coords=discard,
%%%	boxplot/draw direction=y,
%%	%width=\graphwidth,
%%	%height=\graphheight,
%%]
%%%SA
%%\addplot[style={draw=red}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-5-provider-False.csv};
%%\addplot[dotted, style={draw=red}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-5-provider-True.csv};
%%\addplot[style={draw=green}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-10-provider-False.csv};
%%\addplot[dotted, style={draw=green}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-10-provider-True.csv};
%%\addplot[style={draw=blue}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-20-provider-False.csv};
%%\addplot[dotted, style={draw=blue}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-20-provider-True.csv};
%%\addplot[style={draw=black}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-50-provider-False.csv};
%%\addplot[dotted, style={draw=black}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-50-provider-True.csv};
%%\addplot[style={draw=yellow}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-100-provider-False.csv};
%%\addplot[dotted, style={draw=yellow}, line width=1] table [col sep=comma] {sim/SR-graph-pathlength-100-provider-True.csv};
%%\end{axis}
%%\end{tikzpicture}
%%\caption{A plot of the adversarial advantage against sender receiver unlinkability depending on the percentage of compromised mixes. We display one graph per length of the path of mixes. The graphs assume that we have a stratified network topology with $10$ mix nodes per stage and each mix is compromised at random with a probability $p$ equal to the percentage of corruption. The challenge users use different providers (or a compromised provider) (solid lines) or the same uncompromised provider (dotted lines).}\label{fig:compromisedmixplot-sr}
%%
%%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{sections/graphs/security_graph2.pdf}
%\caption{\small{A plot of the adversarial advantage against sender receiver unlinkability depending on the percentage of compromised mixes. We display one graph per length of the path of mixes. The graphs assume that we have a stratified network topology with $10$ mix nodes per stage and each mix is compromised at random with a probability $p$ equal to the percentage of corruption. The challenge users use different providers (or a compromised provider) (solid lines) or the same uncompromised provider (dotted lines).}}
%\label{fig:compromisedmixplot-sr}
%\end{figure}
%
%In \Cref{fig:compromisedmixplot} we show the sender unobservability of \sysname according to \Cref{thm:mixnodeadv}, assuming a stratified network topology with $10$ mix nodes per stage of the network. We plot the adversarial advantage $\delta$ depending on the percentage of corruption of mix nodes. Each line represents an evaluation for a given length of a mix path (from 5 to 100) and we show guarantees both for the case that the users have the \emph{same} (honest) provider and for the case that they have \emph{different} and/or compromised providers. Analogously, in \Cref{fig:compromisedmixplot-sr} we show the sender receiver unlinkability of \sysname according to \Cref{thm:mixnodeadv-sr}.
%
%%\subsection{Active Attacks}
%%
%%Each entity in Loopix (client, mix, provider) maintains self loops to
%%detect active attacks, but how does an entity know when they are under
%%attack and when they simply do not see as many loops as they sent
%%because of congestion in the network? Each entity must choose some
%%parameter, $r$, which is a fraction of the number of loops that are
%%sent, if they do not see this fraction of loops returning they alter
%%their behaviour (e.g. recognize they are being attacked and no longer use the system). We can
%%consider two cases of blocking attacks:
%%\begin{enumerate} 
%%\item The adversary is 
%%targeting a message entering a mix within the internal Loopix network.
%%\item The adversary is targeting a client sending to a provider (on
%%  the edges of Loopix).
%%\end{enumerate}
%%
%%For $(1)$, we consider three sub-cases; (i) when an adversary can
%%perfectly distinguish mix loops from other traffic, (ii) \jamie{is
%%  this a realistic subcase? In other words, when could this happen?} when an
%%adversary can distinguish incoming mix loops from other traffic, but
%%cannot distinguish outgoing loops from other traffic, and (iii) when
%%an adversary cannot distinguish mix loops from other traffic. In (i)
%%an adversary will be able to perform a blocking attack with perfect
%%success, since they are able to distinguish mix loop traffic from user
%%traffic they allow only mix loop traffic and the one message they want
%%to follow in to the mix. The mix will not be aware the attack is
%%taking place since no loops are dropped. The adversary will then
%%follow all messages exiting the mix; the message that eventually is
%%routed to a provider is the message they wish to track since all
%%other messages will not reach the peripheries of the network. In (ii),
%%the message, $m$, that the adversary wishes to track is indistinguishable
%%from outgoing mix loops. The adversary has successfully blocked
%%incoming messages that aren't loops sent by the mix. So there are
%%$\frac{\ell \cdot \lambda_M}{\Delta}$ messages in the
%%messages in the mix at any time. This is the anonymity set for, $m$, the probability of a successful
%%attack is $P(\text{success})=\frac{1}{\frac{\ell \cdot
%%    \lambda_M}{\Delta}+1}=\frac{\Delta}{\ell \cdot \lambda_M +
%%  \Delta}$. In (iii) traffic generated by mix loops is
%%indistinguishable from other traffic. The adversary does not wish to
%%alter the behaviour of the mix (i.e. potentially shutting the mix
%%down), so it can only block mix loops such that $r$ still enter the mix, where
%%$r=\frac{\ell \cdot \lambda_M}{s \cdot \Delta}$, and $s\in\mathbb R_{>
%%    1}$. Since it cannot distinguish loops from other traffic the
%%adversary can do no better than block traffic uniformly such that a
%%fraction $r'$, will be in the mix at any time, where $r'=\frac{k \cdot
%%  \Lambda}{s \cdot \Delta}$. Hence $r'$ is the anonymity set for a
%%message entering a mix and the adversary can do no better than guess
%%at random which was the target message from this set.
%%
%%The probability of successfully tracking a message entering and
%%exiting a mix is dependent on the parameter, $r$. If a mix sets this
%%so they alter their behaviour if they do not see all loops returning,
%%and the adversary cannot distinguish between loops and other traffic,
%%then the adversary cannot launch a blocking attack. However, network
%%congestion may result in dropped messages and the mix erroneously
%%alter their behaviour under the assumption they are being attacked. On
%%the other hand, if a mix sets $r$ such that they do not need any loops
%%to return then adversary is free to block all incoming messages except
%%for the message of interest. However, the message will still belong to an
%%anonymity set of loop messages created at the mix. To recognize when a
%%mix is under attack and provide a large anonymity set we recommend $r$
%%is set somewhere between these two extreme cases.
%%
%%$(2)$ is a simpler setting at the edge of the network. In this
%%scenario Alice sends a message to the provider (after which she is
%%blocked from sending more messages), and all messages from
%%other clients are blocked. Incoming loops entering (and generated by)
%%the provider are distinguishable from client traffic and so the
%%adversary may not block this traffic, hoping not to signal to the
%%provider that they are under attack. This is similar to $(1ii)$, we
%%assume the adversary can see the incoming and outgoing links to a
%%provider and choose to drop traffic, but cannot trivially follow a
%%message throughout the entire network. The adversary can see if an
%%incoming message originated from a mix or a client, and drops all
%%messages that originated from a client. So the provider will only receive: the
%%message that the adversary wishes to track, the loops generated by the
%%provider, and possibly some messages sent to the provider by clients
%%of other providers (note this could be non-loop cover traffic sent by
%%a client). Hence the rate per link to the provider is \jamie{The
%%  amount of traffic to the provider will be the same as normal minus
%%  the loops created by the client. Since the loops created by clients
%%  only reach the internal network. Not sure about this..}: $$ \Lambda' = \frac{(U-j) \cdot ( \ell \cdot
%%    \lambda_P + \ell_C \cdot \lambda_D)}{k \cdot (N+P)}
%%  + \frac{\ell \cdot \lambda_M}{k}$$
%%
%% Where $j$ is the number of blocked
%%  users by the adversary. So the targeted message has $k \cdot \Lambda' / \Delta$ messages as an
%%anonymity set. Of course, the adversary could also block some fraction
%%of incoming messages originating from mixes, up to the fraction at
%%which the provider assumes they are under attack. In other words, they
%%could block traffic such that the anonymity set of the message
%%decreases to $\frac{k \cdot \Lambda'}{s \cdot \Delta}$, where $s\in\mathbb R_{>
%%  1}$.
%%
%%
%%
%
%
%


==> sections/traffic_analysis.tex <==
\section{Traffic Analysis \& Active Attack Resistance}\label{sec:traffic_analysis}

%\begin{xtoc}
%\begin{itemize}
%\item \st{Clients send messages to themselves in loops to generate cover traffic.}
%\item Mixes send messages to themselves to generate cover traffic and detect / mitigate n-1.
%\item Clients, that `know' each other, signal to each others loops of traffic their mutual presence, for presence and to detect partitioning / n-1.
%\item Describe the concrete cryptographic scheme. (How?)
%\item Off-line, on-line protection through synthetic messages from providers, and mitigate end-to-end correlation.
%\item Always-sending model protects against long-term intersection attack.
%\item Sybil-attack?
%\end{itemize}
%\end{xtoc}

% \george{Uses of loops: n-1 attack detection; probing latency of mixes and paths. Friend discovery.}

As described in previous sections, \sysname makes use of a substrate of cover traffic to ensure that messages do not need to be unduly delayed, even when the system does not have a large number of users actively sending messages. 
%Users send cover traffic in the form of \emph{loops}, and \emph{drop} cover traffic as well as a predetermined rate of payload traffic. Mixes, including providers, send their own \emph{loop} cover traffic.
 
The distributions generating all forms of cover and payload traffic are carefully selected. Users send separate streams of Poisson distributed \emph{loops} back to themselves at a rate $\lambda_L$. Each \emph{loop} traverses the user's provider, $\ell$ intermediate mixes selected at random and back to the initial provider. The  dummy cover traffic, generated following a Poisson process with rate $\lambda_D$, passes through the sender's provider and $\ell$ mixes to reach an arbitrarily selected provider, which drops the message. Finally, they emit payload traffic at a Poisson rate of $\lambda_P$. Each message sent by a user is first passed to their provider, next it traverses $\ell$ nodes and a remote provider before being delivered to a final destination. 
The \emph{loop} cover traffic generated by the mixes and providers with rate $\lambda_{M}$ also travels through a path of $\ell$ distinct mixes.

%Users send separate streams of Poisson distributed loops back to themselves at a rate $\lambda_L$, traversing their own provider, $\ell$ intermediate mixes, and then back to their own provider; they also send dummy cover traffic following a Poisson process with rate $\lambda_D$, traversing their own provider, the mix path and being drooped at a random provider, to which it was destinated.  
%and a potentially shorter number of mixes $\ell_C$ until dropped; \ania{we decided to have a cover traffic which traverse to some provider, not that one which is drooped at a random mix node} 
%Finally, they emit payload traffic at a Poisson rate of $\lambda_P$, traversing their provider, $\ell$ mixes, a remote provider before being delivered to a final destination. Mixes and providers generate loops of traffic back to themselves, of length $\ell$. 
 
We remind the reader of some key properties of Poisson processes: aggregating two Poisson processes results in a Poisson process with the sum of their rates, whereas splitting a Poisson processes by selecting messages independently at random into two separate processes results in two Poisson processes with rates proportional to the original rate and the probability of messages being allocated to each separate stream. Finally, Burke's theorem~\cite{burke1956output} states that the the output process of an $M / M / \infty$ queue -- a model for our mixes -- is itself a Poisson process. 

%\jamie{Stratified topology will change the analysis a little, for example: if we assume an stratified topology of the network of providers and mixes, where there are $P$ providers, $N_1$ entry mixes, $N_2$ middle mixes and $N_3$ exit mixes. Let us assume $N_1$=$N_2$=$N_3$, denoted $n$. There are $n$ outgoing links per provider, entry and middle mix. There are $P$ outgoing links per exit mix. So there are $L = (n \cdot P ) \cdot (n^2) \cdot (n^2) \cdot (n \cdot P) = n^6 \cdot P^2$ links in Loopix. Are we set on stratified?}
 
We assume an restricted topology of the network of providers and mixes, and on average $k$ outgoing links are active per node. This results in $L = k \cdot (N+P)$ links in the Loopix system. % \ania{So what is our decision of the topology? In the security proof we so far assume a free-route topology. Maybe we should consider Stratified topology? }

Hence, at any time there should be a traffic rate of $\ell \cdot (\lambda_L + \lambda_P + \lambda_D) / L$ on any link generated by each user, and $\left(\ell \cdot \lambda_{M} \right)/ L$ messages generated by a single mix, leading to an overall Poisson rate per link of 
\begin{align*} 
	\Lambda = \frac{U \cdot  \ell \cdot (\lambda_L + \lambda_P + \lambda_D)}{k \cdot (N+P)} + \frac{\ell \cdot \lambda_M}{k}.
\end{align*}

Each mix having $k$ incoming links, has on average a total rate $k \cdot \Lambda$ of arriving messages. Assuming that the delay in processing those packets is exponentially distributed with parameter $\Delta$, the expected number of messages in each mix at a steady state is $T = k \cdot \Lambda / \Delta$. Thus, we obtain a direct relation between the parameter $T$, representing the number of messages mixed together, the traffic volume on each link $\Lambda$, and the delay at each mix $\Delta$. By injecting additional drop cover traffic $\lambda_D$ and $\lambda_L$ users can collectively maintain a low delay and strong anonymity. However, once the true volume of traffic $\lambda_P$ increases, the lower delay may be maintained at a lower cost by injecting less cover. This approach guarantees that the anonymity properties of \sysname do not come at the cost of performance. 

We now investigate a set of possible active attacks that the adversary might perform to violate the security properties of the system, and show that  \sysname can protect users communication against active adversaries. 




\subsection{Correlation attacks} 
\ania{To be added}
%% \ania{This section has to be fixed!}
%We consider a \emph{correlation attack}, in which an observing adversary tries to identify an outgoing message from a mix, by linking it with an incoming message.  
%In our schema we assume, that the sender of a message includes a delay stamp drawn from an exponential distribution for each hop.  
%Thus, the observation of the message arrival time at the mix does not give an adversary any additional information which might allow to link it to the outgoing packet, as long as there is at least one more message in the mix node queue.  Otherwise, the adversary can correlate the incoming and outgoing message.  
%Thus, the adversary can perform correlation attack if both of the following conditions occur 
%\begin{itemize} 
%        \item at the arrival of a target message, the mix node queue is empty, 
%        \item during the delay time of a target message, no other message arrives, 
%\end{itemize} 
%We denote those two events as $E_{0}, E_{1}$ respectively.  
%The probability of a successful attack is described by a joint probability of those two events. 
%From~\cite{kesdogan1998stop}, we  know that the probability that a server is idle at a steady state when a target message arrives is $\Pr(E_{0}) = e^{\frac{-k\Lambda}{\Delta}}$ and the probability that no other message arrives during the delay time is $\Pr(E_{1}) = \frac{1}{1 + \frac{k\Lambda}{\Delta}}$. Thus, the overall probability of a succeeding attack is 
%\begin{align*} 
%        \Pr(success) = \Pr(E_{0}) \wedge \Pr(E_{1}) = \frac{e^{\frac{-k\Lambda}{\Delta}}}{1 + \frac{k\Lambda}{\Delta}} 
%\end{align*} 
%One can note, that when the traffic rate per link $\Lambda$ increases, the probability of an successful attack decreases. Tunning the mixes cover traffic rate allows us to make the attack probability negligibly small. 


\subsection{Active attacks} 
Instead of simply using noise as a technique to hide traffic patterns, we chose to create
noise messages that loop back to the original sender to provide the ability to detect some forms of active attacks.
We consider blocking attacks at a mix node where an adversary blocks messages entering into a mix in the attempt
to follow some target message when leaving a mix node, referred to as a \emph{mix node (n-1) attack}; we note that similar attacks (and defenses) can be 
applied to a client or provider. We also discuss the success of an adversary
under different capabilities. For the usability of \sysname, it is important that a sender can differentiate 
between an active attack and when they simply do not see as many loops as they send because of congestion in 
the network. We assume that each entity chooses some parameter $r$, which is a fraction of the number of loops that are expected to return
within some time period. If the sender does not see this fraction of loops returning they alter
their behavior (e.g. recognize they are being attacked and no longer use the system).  
  
For a \emph{mix node (n-1) attack}, the adversary could simply block all incoming messages to 
the mix node except a target message, however then the mix node can easily notice that the self 
loops are not returning and deduce that it is under attack. Therefore, an adversary that wants 
to perform a stealthy attack must allow loops to return to the mix node; the adversary must distinguish loop cover traffic
from other types of traffic. We consider three sub-cases of different adversarial advantage: 
\begin{itemize}
	\item[(i)] an adversary is able to perfectly distinguish mix loops from other types of traffic, 
	\item[(ii)] an adversary is able to distinguish incoming loops, but cannot distinguish different types of outgoing traffic, 
	\item[(iii)] an adversary is not able to distinguish any type of traffic.   
\end{itemize}
In the first (i) case, the adversary performs a blocking attack with perfect success, since she is able to distinguish mix loop traffic from user traffic and allows only  mix \emph{loop} traffic and the one message she wants to follow to pass into the mix. The mix will not be aware the attack is taking place since no loops are dropped. The adversary can then observe the target messages exiting the mix. Due to our message packet format and cryptographic primitives we consider this sub-case unrealistic.

In the next scenario (ii) the target message that the adversary wishes to track is indistinguishable 
from the outgoing traffic, including loops. Thus, even if the adversary can perform the attack on the input side, 
there are $\frac{l\cdot \Lambda_{M}}{\Delta}$ loop messages in the mix at any time. Those messages create an anonymity set and so
an adversary can do no better than random guessing among that set. Thus, the probability 
of successful attack is $P(success) = \frac{\Delta}{l \cdot \Lambda_{M} + \Delta}$. One can note, that the bigger the number of mix cover loops, the smaller the probability of a successful attack.  

As with (i), due to our message packet format and cryptographic primitives, the adversary will not be able to  distinguish the \emph{loop} messages from the real and \emph{dummy} messages. We consider the next sub-case to be the most realistic attack.

In (iii) traffic generated by mix loops is indistinguishable from other network traffic.  
The adversary does not wish to alter the behavior of the mix (i.e. potentially shutting the mix down). Thus, the adversary  
has to judicious when blocking messages, to ensure that a fraction $r$ of loops, where $r = \frac{l \cdot \lambda_{M}}{s\cdot \Delta}, 
s\in\mathbb R_{>1}$ return to the mix node\footnote{We give the adversary the advantage of knowing $r$, however in practice this may not be the case.}.
Since the adversary cannot distinguish loops from other traffic the adversary can 
do no better than block traffic uniformly such that a fraction $R$, will be in the mix at any time, 
where $R=\frac{k \cdot \Lambda}{s \cdot \Delta}$. Hence $R$ is the anonymity set for a message entering a mix and the adversary can do no better
than random guessing from this set. 
Following~\cite{danezis2003heartbeat} we estimate how many genuine traffic messages are allowed through to make sure that $r$ loops were not blocked. 
From the negative binomial distribution, we obtain the probability that $x$ real or dummy messages go through before a fraction $r$
of loops are received by the mix. 
Thus, we have
\begin{align*}
	\Pr(X = x) = {x + r' -1 \choose r' }p^{r'} \left( 1 - p\right)^{x},
\end{align*}
where $p$ is the probability of correctly guesing if the message is a loop message or not, $p = \frac{l\cdot \lambda_{M}}{k\cdot \Lambda}$.\jamie{double check this}
% \ania{I think I computed something wrong, since this result does not make sensce for me, can someone check it?}

One can note, that performing $(n-1) - attack$ by blocking (dropping) messages does not give an adversary any significant 
advantage as long as the adversary cannot perfectly distinguish \emph{loop} messages from other types of traffic.  
Motivated by~\cite{kesdogan1998stop}, we now assume that the adversary instead of blocking the messages, can delay all incoming messages for a 
certain amount of time in order to wait until the mix node flushes the target message from the queue after the message delay time has elapsed. 
The adversary needs only make sure that the message is not delayed for too long, because then the mix node discards those messages and it might reveal the attack. 
As shown in~\cite{kesdogan1998stop}, given a timestamp $t$ before which a message must arrive at the mix, the probability of a successful $(n-1) - attack$ is 
\begin{align*} 
        \Pr(success) = \exp{\left(\frac{-k\Lambda \cdot e^{-\Delta \cdot t}}{\Delta}\right)}. 
\end{align*} 
The probability of successful attack decreases exponentially when the traffic rate grows; this value 
has the biggest impact on the probability. This suggests that the cover traffic developed by \sysname can 
protect against $(n-1)-attack$. For a fixed traffic rate, the decreasing exponential parameter $\Delta$ leads 
to a weaker attack. Although the longer messages are delayed from entering a mix, the more powerful the attack becomes, 
this also leads to easier detection of an attack, since many overdue messages would then be dropped by the mix nodes. 


We also note that in a stratified topology, Providers are able to distinguish \emph{loop} messages sent by mix nodes from
other types of traffic. However, we do not consider this to be a substantial attack vector since (i) Providers are assumed
honest but curious, and are afforded more trust than regular mix nodes, (ii) \emph{loop} messages sent by mix nodes are evenly
distributed among all Providers, reducing the risk that a large amount of a target mix node loops are routed through a 
corrupt Provider, (iii) Providers do not learn the which mix node sent the \emph{loop} since Sphinx removes the ability to
infer a messages position in a path.

\subsection{Anonymity Set}

%\george{DO: We can claculate the relation of rate of cover traffic, to
 % rate of delay to target specific anonymity guarantees at mixes.}
%\jamie{ ( Someone please check my work, a lot of symbols, mistakes may
 % have been made ). }
  
Quantifying the relationship between rate of total cover traffic in Loopix and rate of delay of a message - we have that the expected number of messages in a mix at any time (as long as rates don't change) is: $T = k \cdot \Lambda / \Delta$ and rate of messages per link is: 
\begin{align*}
	\Lambda = \frac{U \cdot ( \ell \cdot (\lambda_L + \lambda_P) + \ell_C \cdot \lambda_D)}{k \cdot (N+P)} + \frac{\ell \cdot \lambda_M}{k}.
\end{align*}
Suppose we want there to be more than $n$ messages in any mix at any time. Then we require $T \geq n$, thus we require:
\begin{align*}
	n \cdot \Delta \leq \frac{U \cdot ( \ell \cdot  (\lambda_L + \lambda_P) + \ell_C \cdot \lambda_D)}{ (N+P)} + \ell \cdot \lambda_M
\end{align*}
Separating cover traffic terms from rate of delay we have: 
\begin{align*}
	&n \Delta (N+P) - \ell \cdot U \lambda_P  \\
	&\quad \leq U (\ell \cdot \lambda_L + \ell_C \cdot \lambda_D) + (N+P) \cdot  \ell \cdot \lambda_M
\end{align*}


%\begin{xtoc}
%\begin{itemize}
%\item Analysis of unlinkability: crappy metrics (adhoc) all the way to Bayesian metrics (Troncoso et al -- complex.)
%\item Estimation of success of attack, and over how much time, and under what adversary condition and volume of cover traffic.
%\item Cover traffic volume vs. anonymity.
%\item (n-1) attack: analysis of susceptibility, volume of Green traffic under different types of attack; success in detecting attack under different volumes of Red traffic. Effectiveness of Loops.
%\item Susceptibility to end-to-end attacks / fingerprinting (class of service, etc).
%\item Long term attack: effectiveness of cover / Providers in mitigating. How much time? Can we have a theorem?
%\item Defense against weaker threat models -- comprise with Tor / Onion Routing.
%\end{itemize}
%\end{xtoc}

%We assume the topology of the network of providers and mixes is restricted, and on average $k$ outgoing links are active per node. This results in $L = k \cdot (N+P)$ links in the Loopix system. 
%
%If we have $L$ links then at any time there should be a rate of $(\ell \cdot (\lambda_L + \lambda_P) + \ell_C \cdot \lambda_D ) / L$ traffic on any link from one user, and $\ell \cdot \lambda_M / L$ per mix, leading to an overall Poisson rate per link of:
%$$ \Lambda = \frac{U \cdot ( \ell \cdot (\lambda_L + \lambda_P) + \ell_C \cdot \lambda_D)}{k \cdot (N+P)} + \frac{\ell \cdot \lambda_M}{k}$$
%
%The average mix will have $k$ incoming links, and the total rate of arrivals of messages will be on average $k \cdot \Lambda$. Assuming the delay in processing those is exponentially distributed with parameter $\Delta$, the expected number of messages in each mix at a steady state is: $T = k \cdot \Lambda / \Delta$. There is thus a direct relation between the parameter $T$, representing the number of messages mixed together, the traffic volume on each link $\Lambda$, and the delay at each mix $\Delta$. By injecting additional drop cover traffic $\lambda_D$ and $\lambda_L$ users can collectively maintain a low delay and good anonymity. However, once the true volume of traffic $\lambda_P$ increases, the lower delay may be maintained at a lower cost by injecting less cover.
%
%\jamie{Possible Attacks on sg-mixes based on what George wrote and how Loopix can defend against them:}
%
%\jamie{- Correlation Attack - an attacker can correlate the incoming and outgoing of a message in a mix if during the delay time no other message is in the queue. The probability that there are no other messages in the mix at the time of a new message arrival is $e^{\frac{-k \cdot \Lambda}{\Delta}}$. The probability that no other messages arrive while the message is delayed in the mix is $\frac{\Delta}{(k \cdot \Lambda) + \Delta}$. The overal probability of a successful correlation attack is joint probability of these two event, since they are independent, the probability of a successful attack is $\frac{e^{\frac{-k \cdot \Lambda}{\Delta}}}{1+\frac{k \cdot \Lambda}{\Delta}}$. This probability made negligibly small by the tuning the mixes cover rate traffic.}
%
%\jamie{- n-1 attack: Details to be added later - given a time window $t$ in which a message must arrive at the mix, the probability of a successful n-1 attack is $exp(\frac{-k \cdot \Lambda \cdot e^{-\Delta \cdot t}}{\Delta})$}




